Grid Generation and Adaptation by Functionals

Accuracy of a simulation is strongly depend on the grid quality. Here, quality means orthogonality at the boundaries and quasi-orthogonality within the critical regions, smoothness, bounded aspect ratios, solution adaptive behaviour, etc. We review various functionals for generating high quality structured quadrilateral meshes in two dimensional domains. Analysis of Winslow and Modified Liao functionals are presented. Numerical examples are also presented to support our theoretical analysis. We will demonstrate the use of the Area functional for generating adaptive quadrilateral meshes.

==> Makefile <==
# Generic make file for LaTeX: requires GNU make
#
# This makefile provides four targets: dvi, ps, pdf and clean.
# The default is "pdf".
# To make a dvi file, type "make dvi"
# To make a ps file, type "make ps".
# To make a pdf file, type "make pdf" or simply "make".
# To remove all files generated by make, type "make clean".
#
# Rouben Rostmaian
# September 2002

TEXFILE =     article.tex
#TEXFILE	= slides.tex

.PHONY: dvi ps pdf clean

pdf:	$(TEXFILE:.tex=.pdf)
ps:	$(TEXFILE:.tex=.ps)
dvi:	$(TEXFILE:.tex=.dvi)

%.dvi: %.tex
	( \
	\latex $<; \
	while \grep -q "Rerun to get cross-references right." $(<:.tex=.log); \
	do \
		\latex $<; \
	done \
	)

%.ps: %.dvi
	\dvips -q -t a4 $<

%.pdf: %.ps
	\ps2pdf -dPDFSETTINGS=/prepress $<

clean:
	@\rm -f \
	$(TEXFILE:.tex=.aux) \
	$(TEXFILE:.tex=.log) \
	$(TEXFILE:.tex=.out) \
	$(TEXFILE:.tex=.dvi) \
	$(TEXFILE:.tex=.ps)

